Exploiting Multiple Representations: 3D Face Biometrics Fusion with Application to Surveillance

3D face reconstruction (3DFR) algorithms are based on specific assumptions tailored to the limits and characteristics of the different application scenarios. In this study, we investigate how multiple state-of-the-art 3DFR algorithms can be used to generate a better representation of subjects, with the final goal of improving the performance of face recognition systems in challenging uncontrolled scenarios. We also explore how different parametric and non-parametric score-level fusion methods can exploit the unique strengths of multiple 3DFR algorithms to enhance biometric recognition robustness. With this goal, we propose a comprehensive analysis of several face recognition systems across diverse conditions, such as varying distances and camera setups, intra-dataset and cross-dataset, to assess the robustness of the proposed ensemble method. The results demonstrate that the distinct information provided by different 3DFR algorithms can alleviate the problem of generalizing over multiple application scenarios. In addition, the present study highlights the potential of advanced fusion strategies to enhance the reliability of 3DFR-based face recognition systems, providing the research community with key insights to exploit them in real-world applications effectively. Although the experiments are carried out in a specific face verification setup, our proposed fusion-based 3DFR methods may be applied to other tasks around face biometrics that are not strictly related to identity recognition.

==> Tables/cross_table_complete.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Average results in the cross-setting context} considering both different acquisition distance and camera between training and test set. For each metric and verification system (based on XceptionNet and AdaFace), we highlight the best result achieved when enhanced through the single 3DFR algorithm (3DDFA v2, EOS, NextFace, and HRN) and the best result obtained through each score-level fusion approach (non-parametric fusion rules, weighted averages, and classification models).}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc|ccccc|}
\cline{2-11}
 &
  \multicolumn{5}{|c|}{\textbf{XceptionNet-based \cite{chollet2017xception}}} &
  \multicolumn{5}{c|}{\textbf{AdaFace \cite{kim2022adaface}}  }\\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Method}}} &
  \textbf{AUC}&
  \textbf{EER} &
  \textbf{Cohen's} &
  \textbf{\%FMR at} &
  \textbf{\%FNMR at} &
  \textbf{AUC} &
  \textbf{EER} &
  \textbf{Cohen's} &
  \textbf{\%FMR at} &
  \textbf{\%FNMR at}  \\
\multicolumn{1}{|c|}{} &
   \textbf{{[}\%{]}} &
   \textbf{{[}\%{]}} &
  \textbf{d} &
  \textbf{FNMR=1\%} &
  \textbf{FMR=1\%} &
   \textbf{{[}\%{]}} &
   \textbf{{[}\%{]}} &
  \textbf{d} &
  \textbf{FNMR=1\%} &
  \textbf{FMR=1\%}  \\ \hline
\multicolumn{1}{|c|}{\textbf{Baseline}} &
  68.97 &
  36.21 &
  0.63 &
  91.81 &
  96.53  &
  96.95 &
  8.42 &
  2.89 &
  47.40 &
  34.51  \\ \hline
\multicolumn{1}{|c|}{\textbf{3DDFA v2 \cite{guo2020towards}}} &
  70.95 &
  19.70 &
  \textbf{0.69} &
  96.22 &
  92.53 &
  97.05 &
  0.53 &
  3.19 &
  26.91 &
  26.82  \\
\multicolumn{1}{|c|}{\textbf{EOS \cite{eos}}} &
  \textbf{71.21} &
  \textbf{19.09} &
  0.61 &
  96.57 &
  \textbf{91.58}  &
  \textbf{97.26} &
  \textbf{0.12} &
  \textbf{3.34} &
  \textbf{23.63} &
  \textbf{22.25}  \\
\multicolumn{1}{|c|}{\textbf{NextFace \cite{dib2021practical}}} &
  68.47 &
  23.46 &
  0.57 &
  95.99 &
  94.97 &
  94.15 &
  3.57 &
  2.35 &
  40.67 &
  48.40 
   \\ 
  \multicolumn{1}{|c|}{\textbf{HRN \cite{lei2023hierarchical}}} &
  66.94 &
  22.25 &
  0.48 &
  \textbf{94.82} &
  95.63 &
  97.12 &
  1.05 &
  3.24 &
  25.44 &
  25.77  \\\hline
\multicolumn{1}{|c|}{\textbf{Min}} &
  81.08 &
  23.40 &
  0.87 &
  85.46 &
  85.28 &
  97.71 &
  0.31 &
  3.44 &
  22.29 &
  22.23  \\
\multicolumn{1}{|c|}{\textbf{Max}} &
  83.33 &
  21.83 &
  \textbf{1.39} &
  63.58 &
  90.89 &
  97.72 &
  0.12 &
  3.24 &
  19.88 &
  23.61  \\
  \multicolumn{1}{|c|}{\textbf{Prod}} &
  \textbf{84.45} &
  18.72 &
  1.37 &
  \textbf{60.90} &
  \textbf{84.34} &
  98.54 &
  0.12 &
  3.68 &
  \textbf{13.74} &
  16.50  \\ 
  \multicolumn{1}{|c|}{\textbf{Avg}} &
  75.77 &
  \textbf{16.44} &
  0.86 &
  83.41 &
  89.84 &
  \textbf{98.55} &
  \textbf{0.06} &
  3.80 &
  13.78 &
  \textbf{16.34}  \\
\multicolumn{1}{|c|}{\textbf{Bayesian Avg}} &
  77.03 &
  26.65 &
  0.90 &
  80.96 &
  89.72 &
  98.54 &
  \textbf{0.06} &
  \textbf{4.00} &
  \textbf{13.74} &
  16.45  \\
  
  \hline
  \multicolumn{1}{|c|}{\textbf{PCC-based Avg}} &
  76.95 &
  26.81 &
  0.92 &
  81.01 &
  89.94 &
  98.54 &
  \textbf{0.06} &
  \textbf{4.00} &
  \textbf{13.74} &
  16.45  \\
  \multicolumn{1}{|c|}{\textbf{MI-based Avg}} &
  \textbf{85.29} &
  18.98 &
  \textbf{1.39} &
  61.27 &
  85.32  &
  \textbf{98.55} &
  \textbf{0.06} &
  3.80 &
  13.78 &
  16.32  \\
  \multicolumn{1}{|c|}{\textbf{Acc-based Avg}} &
  85.26 &
  \textbf{18.92} &
  \textbf{1.39} &
  \textbf{61.06} &
  \textbf{84.15}  &
  \textbf{98.55} &
  \textbf{0.06} &
  3.81 &
  13.75 &
  \textbf{16.31}  \\
 \hline
 \multicolumn{1}{|c|}{\textbf{SVM}} &
  78.62 &
  22.11 &
  1.20 &
  82.16 &
  96.94  &
  97.31 &
  0.12 &
  3.73 &
  24.88 &
  18.70  \\
  \multicolumn{1}{|c|}{\textbf{MLP}} &
  \textbf{83.34} &
  \textbf{19.78} &
  \textbf{1.48} &
  \textbf{65.58} &
  \textbf{85.09}  &
  \textbf{98.54} &
  \textbf{0.06} &
  \textbf{7.78} &
  \textbf{13.84} &
  \textbf{16.13}  \\
  \multicolumn{1}{|c|}{\textbf{Perceptron}} &
  75.97 &
  27.36 &
  0.95 &
  82.28 &
  90.64  &
  98.51 &
  \textbf{0.06} &
  7.62 &
  14.06 &
  16.37  \\
\hline
\end{tabular}%
}
\label{tab:crossRGB_complete}
\end{table*}

==> Tables/intra_table_complete.tex <==
\begin{table*}[h]
\centering
\caption{\textbf{Average results in the intra-setting context.} For each metric and verification system (based on VGG19, XceptionNet, MobileNet V3, and AdaFace), we highlight the best result achieved when enhanced through the single 3DFR algorithm (3DDFA v2, EOS, NextFace, and HRN) and the best result obtained through each score-level fusion approach (non-parametric fusion rules, weighted averages, and classification models).}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc|ccccc|}
\cline{2-11}
 &
  \multicolumn{5}{|c|}{\textbf{VGG19-based \cite{simonyan2014very} }} &
  \multicolumn{5}{c|}{\textbf{XceptionNet-based \cite{chollet2017xception}}}  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Method}}} &
  \textbf{AUC} &
  \textbf{EER} &
  \textbf{Cohen's} &
  \textbf{\%FMR at} &
  \textbf{\%FNMR at} &
  \textbf{AUC} &
  \textbf{EER} &
  \textbf{Cohen's} &
  \textbf{\%FMR at} &
  \textbf{\%FNMR at}  \\
\multicolumn{1}{|c|}{} &
   \textbf{{[}\%{]}} &
   \textbf{{[}\%{]}} &
  \textbf{d} &
  \textbf{FNMR=1\%} &
  \textbf{FMR=1\%} &
   \textbf{{[}\%{]}} &
   \textbf{{[}\%{]}} &
  \textbf{d} &
  \textbf{FNMR=1\%} &
  \textbf{FMR=1\%}  \\ \hline
 \multicolumn{1}{|c|}{\textbf{Baseline}} &
  75.56 &
  29.31 &
  0.94 &
  87.31 &
  87.03 &
  76.03 &
  25.86 &
  0.89 &
  83.93 &
  90.91  \\ \hline
\multicolumn{1}{|c|}{\textbf{3DDFA v2 \cite{guo2020towards}}} &
  81.56 &
  20.94 &
  1.07 &
  74.93 &
  \textbf{90.69} &
  80.35 &
  24.38 &
  1.02 &
  \textbf{79.05} &
  \textbf{89.01}  \\
\multicolumn{1}{|c|}{\textbf{EOS \cite{eos}}} &
  80.63 &
  22.11 &
  1.02 &
  81.12 &
  95.04 &
  \textbf{81.55} &
  \textbf{22.29} &
  \textbf{1.07} &
  83.07 &
  89.45  \\
\multicolumn{1}{|c|}{\textbf{NextFace \cite{dib2021practical}}} &
  74.02 &
  27.21 &
  0.80 &
  71.18 &
  95.72 &
  76.16 &
  26.79 &
  0.83 &
  86.15 &
  93.47 
   \\ 
  \multicolumn{1}{|c|}{\textbf{HRN \cite{lei2023hierarchical}}} &
  \textbf{83.21} &
  \textbf{19.97} &
  \textbf{1.17} &
  \textbf{68.86} &
  92.01 &
  80.47 &
  23.83 &
  1.02 &
  80.86 &
  89.70  \\\hline
  \multicolumn{1}{|c|}{\textbf{Min}} &
  85.38 &
  18.42 &
  0.93 &
  87.49 &
  89.30 &
  81.08 &
  23.40 &
  0.87 &
  85.46 &
  85.28  \\
\multicolumn{1}{|c|}{\textbf{Max}} &
  77.01 &
  23.36 &
  1.18 &
  64.47 &
  93.87 &
  83.33 &
  21.83 &
  \textbf{1.39} &
  63.58 &
  90.89  \\
\multicolumn{1}{|c|}{\textbf{Prod}} &
  \textbf{87.87} &
  \textbf{18.41} &
  1.59 &
  \textbf{49.97} &
  85.45 &
  \textbf{85.45} &
  \textbf{18.72} &
  1.37 &
  \textbf{60.90} &
  \textbf{84.34}  \\
  \multicolumn{1}{|c|}{\textbf{Avg}} &
  87.35 &
  18.78 &
  \textbf{1.60} &
  50.76 &
  \textbf{84.75} &
  85.22 &
  19.05 &
  \textbf{1.39} &
  61.15 &
  \textbf{84.34}  \\
\multicolumn{1}{|c|}{\textbf{Bayesian Avg}} &
  85.92 &
  21.86 &
  1.43 &
  56.23 &
  86.26 &
  85.13 &
  18.92 &
  1.38 &
  61.04 &
  84.85  \\
  
  
 \hline
 \multicolumn{1}{|c|}{\textbf{PCC-based Avg}} &
    \textbf{87.43} &
    \textbf{18.65} &
    1.59  &
    49.51 &
    \textbf{84.59} &
    \textbf{85.39} &
    \textbf{18.58} &
    \textbf{1.39} &
    \textbf{60.80} &
    85.07 \\
   \multicolumn{1}{|c|}{\textbf{MI-based Avg}} &
  87.33 &
  19.03 &
  1.57 &
  \textbf{49.41} &
  85.70 &
  85.29 &
  18.98 &
  \textbf{1.39} &
  61.27 &
  85.32  \\
 \multicolumn{1}{|c|}{\textbf{Acc-based Avg}} &
  87.38 &
  18.66 &
  \textbf{1.60} &
  50.46 &
  84.98 &
  85.26 &
  18.92 &
  \textbf{1.39} &
  61.06 &
  \textbf{84.15}  \\ \hline
\multicolumn{1}{|c|}{\textbf{SVM}} &
  79.87 &
  20.87 &
  1.27 &
  72.88 &
  94.62 &
  78.62 &
  22.11 &
  1.20 &
  82.16 &
  96.94  \\ 
\multicolumn{1}{|c|}{\textbf{MLP}}&
  85.07 &
  18.84 &
  \textbf{1.54} &
  \textbf{59.11} &
  87.72 &
  \textbf{83.34} &
  19.78 &
  \textbf{1.48} &
  \textbf{65.58} &
  \textbf{85.09}  \\
  \multicolumn{1}{|c|}{\textbf{Perceptron}} &
  \textbf{85.83} &
  \textbf{17.80} &
  1.52 &
  58.03 &
  \textbf{87.16} &
  83.09 &
  \textbf{19.11} &
  1.45 &
  69.85 &
  87.21  \\
\hline
  
 \\ \cline{2-11}
  &
  \multicolumn{5}{|c|}{\textbf{MobileNet-based \cite{mobilenetv3}}} &
  \multicolumn{5}{c|}{\textbf{AdaFace \cite{kim2022adaface}}}  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Method}}} &
  \textbf{AUC} &
  \textbf{EER} &
  \textbf{Cohen's} &
  \textbf{\%FMR at} &
  \textbf{\%FNMR at} &
  \textbf{AUC} &
  \textbf{EER} &
  \textbf{Cohen's} &
  \textbf{\%FMR at} &
  \textbf{\%FNMR at}  \\
\multicolumn{1}{|c|}{} &
   \textbf{{[}\%{]}} &
   \textbf{{[}\%{]}} &
  \textbf{d} &
  \textbf{FNMR=1\%} &
  \textbf{FMR=1\%} &
   \textbf{{[}\%{]}} &
   \textbf{{[}\%{]}} &
  \textbf{d} &
  \textbf{FNMR=1\%} &
  \textbf{FMR=1\%}  \\ \hline
  \multicolumn{1}{|c|}{\textbf{Baseline}} &
  61.50 &
  50.00 &
  0.38 &
  93.65 &
  94.03 &
  93.09 &
  5.30 &
  2.99 &
  28.32 &
  30.21  \\ \hline
\multicolumn{1}{|c|}{\textbf{3DDFA v2 \cite{guo2020towards}}} &
  51.10 &
  \textbf{50.00} &
  0.10 &
  96.88 &
  98.83 &
  97.98 &
  2.89 &
  3.49 &
  \textbf{14.88} &
  20.06  \\
\multicolumn{1}{|c|}{\textbf{EOS \cite{eos}}} &
  49.97 &
  \textbf{50.00} &
  0.10 &
  97.23 &
  \textbf{98.37} &
  \textbf{98.25} &
  \textbf{1.91} &
  \textbf{3.67} &
  17.44 &
  \textbf{17.01}  \\
\multicolumn{1}{|c|}{\textbf{NextFace \cite{dib2021practical}}} &
  \textbf{52.48} &
  \textbf{50.00} &
  0.10 &
  97.70 &
  98.58 &
  96.04 &
  8.31 &
  2.69 &
  33.33 &
  35.02 
   \\ 
  \multicolumn{1}{|c|}{\textbf{HRN \cite{lei2023hierarchical}}} &
  51.94 &
  \textbf{50.00} &
  \textbf{0.13} &
  \textbf{96.47} &
  98.81 &
  97.99 &
  3.39 &
  3.54 &
  17.62 &
  19.83  \\\hline
  \multicolumn{1}{|c|}{\textbf{Min}} &
  51.11 &
  \textbf{50.00} &
  0.10 &
  97.52 &
  99.52 &
  98.42 &
  2.51 &
  3.79 &
  16.47 &
  15.57  \\
\multicolumn{1}{|c|}{\textbf{Max}} &
  \textbf{53.01} &
  \textbf{50.00} &
  \textbf{0.15} &
  \textbf{95.42} &
  99.30 &
  98.47 &
  1.97 &
  3.64 &
  12.69 &
  15.73  \\
\multicolumn{1}{|c|}{\textbf{Prod}} &
  51.25 &
  \textbf{50.00} &
  0.09 &
  96.72 &
  \textbf{99.28} &
  98.98 &
  0.80 &
  4.05 &
  10.30 &
  11.00  \\ 
  \multicolumn{1}{|c|}{\textbf{Avg}} &
  51.25 &
  \textbf{50.00} &
  0.09 &
  96.72 &
  \textbf{99.28} &
  \textbf{98.99} &
  \textbf{0.68} &
  \textbf{4.18} &
  \textbf{10.07} &
  \textbf{10.54}  \\
  \multicolumn{1}{|c|}{\textbf{Bayesian Avg}} &
  50.00 &
  \textbf{50.00} &
  0.00 &
  100.00 &
  100.00 &
  \textbf{98.99} &
  \textbf{0.68} &
  \textbf{4.18} &
  \textbf{10.07} &
  \textbf{10.54}  \\
  
 \hline
  \multicolumn{1}{|c|}{\textbf{PCC-based Avg}} &
    \textbf{51.52} &
    \textbf{50.00} &
    0.07  &
    97.75 &
    98.33 &
    \textbf{99.00} &
    \textbf{0.68} &
    \textbf{4.20} &
    \textbf{9.92} &
    10.77 \\
  \multicolumn{1}{|c|}{\textbf{MI-based Avg}} &
  51.34 &
  \textbf{50.00} &
  \textbf{0.11} &
  \textbf{96.71} &
  \textbf{98.82} &
  98.99 &
  \textbf{0.68} &
  4.18 &
  10.05 &
  \textbf{10.54}  \\
   \multicolumn{1}{|c|}{\textbf{Acc-based Avg}} &
  51.25 &
  \textbf{50.00} &
  0.10 &
  96.72 &
  99.28 &
  \textbf{99.00} &
  \textbf{0.68} &
  4.19 &
  10.05 &
  \textbf{10.54}  \\ \hline

\multicolumn{1}{|c|}{\textbf{SVM}} &
  \textbf{50.83} &
  \textbf{43.90} &
  \textbf{0.17} &
  \textbf{97.42} &
  98.85 &
  98.11 &
  3.20 &
  4.32 &
  19.62 &
  14.37  \\ 
\multicolumn{1}{|c|}{\textbf{MLP}} &
  50.07 &
  50.00 &
  0.10 &
  97.71 &
  \textbf{99.52} &
  \textbf{98.99} &
  0.92 &
  \textbf{9.08} &
  10.32 &
  \textbf{10.31}  \\
 \multicolumn{1}{|c|}{\textbf{Perceptron}} &
  50.17 &
  50.00 &
  0.15 &
  97.52 &
  99.77 &
  98.95 &
  \textbf{0.80} &
  8.93 &
  \textbf{10.01} &
  10.78  \\
  
 \hline
\end{tabular}%
}
\label{tab:intraRGB_complete}
\end{table*}
